DispersedLedger: High-Throughput Byzantine Consensus on Variable Bandwidth Networks

The success of blockchains has sparked interest in large-scale deployments of Byzantine fault tolerant (BFT) consensus protocols over wide area networks. A central feature of such networks is variable communication bandwidth across nodes and across time. We present DispersedLedger, an asynchronous BFT protocol that provides near-optimal throughput in the presence of such variable network bandwidth. The core idea of DispersedLedger is to enable nodes to propose, order, and agree on blocks of transactions without having to download their full content. By enabling nodes to agree on an ordered log of blocks, with a guarantee that each block is available within the network and unmalleable, DispersedLedger decouples bandwidth-intensive block downloads at different nodes, allowing each to make progress at its own pace. We build a full system prototype and evaluate it on real-world and emulated networks. Our results on a geo-distributed wide-area deployment across the Internet shows that DispersedLedger achieves 2x better throughput and 74% reduction in latency compared to HoneyBadger, the state-of-the-art asynchronous protocol.

==> apps.tex <==
\section{\redstrike{Application Scenarios} \red{Sharding DispersedLedger}
\label{sec:applications}


\textbf{Sharding} Each node takes a small shard of ledger.








==> design.tex <==
\section{Design}

\subsection{System Model}




\subsection{Overview}

Inspired by HoneyBadger, DispersedLedger runs in epochs, where each epoch commits roughly $N$ blocks (1 block per node), which contain transactions submitted by clients. As in HoneyBadger, transactions submitted by clients are stored in each node's input buffer. At the beginning of each epoch, each node packs transactions in its input buffer as a block and proposes it to be committed in the current epoch.

Unlike HoneyBadger, DispersedLedger does not broadcast its proposal blocks; rather, it \textit{disperse} the content of proposal blocks to the entire cluster. Through Verifiable Information Dispersal (VID, our first building block), a node can ensure the availability of the proposal block content for later retrievals in spite of $f$ byzantine failures; by leveraging cryptography, VID ensures availability after transferring much less data than reliable broadcasts.

DispersedLedger relies on Binary Agreement (BA) to reach a consensus on which proposal blocks are successfully dispersed and thus should be committed in the current epoch. Such agreements are necessary since we cannot wait for all blocks to be dispersed. Some of $f$ byzantine nodes may have not invoked \texttt{Dispersal}(B, K) or sent \textit{Chunk} only to a few nodes. With BA, we irreversibly exclude those blocks from the current epoch.

The blocks determined to be committed can be retrieved lazily without stopping epochs from proceeding. The asynchronous retrieval of blocks allows each node to adapt to temporal network bandwidth variations without slowing down other nodes with enough network bandwidth.

\subsection{Building Block 1: VID}


\subsubsection{Model}
\label{sec:avid-model}
The first building block of DispersedLedger is \textit{Verifiable Information Dispersal} (VID)~\cite{avid}. It allows clients to store data across $N$ servers and later download the data from the servers, in spite of $f (\le \frac{N-1}{3})$ byzantine servers. In our use case, each DispersedLedger node serves as both a client and server for VID.

VID has two primitives: \texttt{Dispersal}$(B, K)$ which stores a block $B$ across the cluster with the key $K$, and \texttt{Retrieval}$(\text{\red{invoker\_id}}, K)$ which queries the cluster for the contents of the block $B$ by its key $K$ \red{and the indentifier of the node that dispersed $B$}.

An VID protocol must provide the following properties on an asynchronous network with high probability~\cite{avid}:
\begin{itemize}
    \item \textbf{Termination}: If a correct client initiates the dispersal of a block $B$ with a key $K$, all honest servers eventually complete the dispersal. 
    \item \textbf{Agreement}: If some correct server has completed a dispersal $K$, all correct servers eventually complete the dispersal.
    \item \textbf{Availability}: If a dispersal $K$ completes on a correct server, and a correct client starts the retrieval protocol for $K$, it eventually reconstructs some block $B'$.
    \item \textbf{Correctness}: If the dispersal of a block $B$ completes on a correct server, all correct clients reconstruct the same block $B'$ by running the retrieval protocol. Also, if the dispersal was initiated by a correct client, then $B=B'$.
\end{itemize}

\subsubsection{AVID-M Protocol}
We developed a new VID protocol on asynchronous network, Asynchronous Verifiable Information Dispersal with Merkle-tree (AVID-M). Our protocol is more efficient than the previous state of the art, AVID-FP~\cite{avidfp}.

AVID-M achieves VID by encoding a block $B$ using an $(N-2f, N)$-erasure code; the erasure coding scheme generates $N$ chunks, and the original block can be recovered just from $N-2f$ chunks.

\textbf{Dispersal algorithm} is formally defined in  Figure~\ref{fig:dispersalAlgo}. %

A client begins a dispersal by encoding the block $B$ using an $(N-2f, N)$-erasure code. It then sends each of the $N$ chunks to each of the $N$ servers. However, those dispersed chunks may get forged by byzantine nodes. We use Merkle proof~\cite{merkle} to allow other correct nodes or retriever to detect any forgery on the dispersed chunks. \red{more explanation? maybe in appendix?}

When a server receives its chunk from the client, it notifies other nodes by sending \texttt{GotChunk}. Once a server gets $N-f$ \texttt{GotChunk} messages, it knows that at least $N-2f$ chunks have reached \textit{correct} servers, which are enough for later retrieval; so, the server broadcasts a \texttt{Ready} message.

\texttt{Ready} messages are necessary to ensure all other correct servers will also terminate the dispersal before a server with $N-2f$ \texttt{GotChunk} messages can terminate. If the invoker of dispersal was not byzantine, we don't need \texttt{Ready} messages as all correct nodes will be able to receive $N-2f$ \texttt{GotChunk} messages as well. However, if the dispersal invoker was malicious, it could send \texttt{Chunk} to only $N - 2f$ correct nodes. Then, $f$ byzantine nodes may send \texttt{GotChunk} only to one correct server. In that case, only one of correct nodes will terminate the dispersal. 

Instead of immediately terminating the dispersal, servers form a consensus on the termination. After collecting $f+1$ \texttt{Ready} messages, a server knows at least one correct server confirmed the distribution of chunks to enough correct nodes (i.e., the block will be available for retrieval). So, the server spread the word about the chunk distribution by broadcasting \textit{Ready} messages even if it didn't collect enough \texttt{GotChunk} messages. Once a server collects \textit{Ready} messages from $2f+1$ servers, it knows other servers will also get $2f+1$ \textit{Ready} messages, so it can terminate with agreement. More details on this reasoning is in \S\ref{sec:avidm-correctness}

\begin{figure}
\centering
\fbox{%
  \parbox{0.95\columnwidth}{%

\underline{\textbf{\texttt{Dispersal}(B,K) invoker}}
\vspace{2pt}
\begin{enumerate}
    \item Encode the input block $B$ using an $(N-2f, N)$-erasure code, which results in N chunks, $\{C_i\}_{i \in (1,2, .., N)}$.
    \item Form a Merkle-tree with all chunks $\{C_i\}_{i \in (1,2, .., N)}$, and calculate the Merkle-tree root, $r$.
    \item Send \texttt{Chunk}$(K, r, C_i, P_i)$ to the $i$-th server. Here $P_i$ is the $i$-th Merkle proof.
\end{enumerate}

\vspace{10pt}

\underline{\textbf{\texttt{Dispersal}(B,K) handler for $i$-th node}}
\vspace{2pt}
\begin{itemize}
    \item Upon receiving \texttt{Chunk}$(K, r, C_i, P_i)$:
    \begin{enumerate}
        \item Check if the Merkle proof $P_i$ matches the chunk $C_i$ and the root $r$. If not, ignore the message.
        \item Save \texttt{Chunk}$(K, r, C_i, P_i)$ durably.
        \item Set the counter $\text{ValidShareCount}[K] = 1$.
        \item Set the counter $\text{ReadyCount}[K] = 0$.
        \item Broadcast \texttt{GotChunk}$(K, r)$.
    \end{enumerate}
    \item Upon receiving \texttt{GotChunk}$(K, r)$ from the $j$-th node:\footnote{Assume that a server buffers all messages related to a key $K$ which it has not received a corresponding \texttt{Chunk} message.}
    \begin{enumerate}
        \item Check if $r$ is the same as the one previously received in the \texttt{Chunk} message. If not, ignore the message.
        \item If it is the first \texttt{GotChunk}$(K, r)$ message from the $j$-th node, increment $\text{ValidShareCount}[K]$.
        \item If $\text{ValidShareCount}[K] \ge N-f$, broadcast \texttt{Ready}$(K)$.
    \end{enumerate}
    \item Upon receiving \textit{Ready}$(K)$ from the $j$-th node (including the server itself):
    \begin{enumerate}
        \item If it is the first \texttt{Ready}$(K)$ message from the $j$-th node, increment $\text{ReadyCount}[K]$.
        \item If $\text{ReadyCount}[K] \ge f+1$, broadcast \texttt{Ready}$(K)$ if not done so.
        \item If $\text{ReadyCount}[K] \ge 2f+1$, terminate.
    \end{enumerate}
\end{itemize}
} }
\caption{
Algorithm for \texttt{Dispersal}(B, K)
}
\label{fig:dispersalAlgo}
\end{figure}

\begin{figure}
\centering
\fbox{%
  \parbox{0.95\columnwidth}{%

\underline{\textbf{\texttt{Retrieval}(K, r) invoker}}
\vspace{2pt}
\begin{itemize}
    \item Broadcast \texttt{RequestChunk}$(K, r)$ to all nodes.
    \item Upon receiving \texttt{ReturnChunk}$(K, r, C_i, P_i)$ from the $i$-th server:
    \begin{enumerate}
        \item Check that the Merkle proof $P_i$ matches the root $r$ and the chunk $C_i$. If not, ignore the messsage.
        \item Save the chunk.
    \end{enumerate}
    \item Upon collecting $N-2f$ or more different chunks for the block:
    \begin{enumerate}
        \item Decode using any $N-2f$ chunks collected to recover a block $B'$.
        \item Encode the block $B'$ using the same erasure code to get chunks $\{C_i'\}_{i \in [N]}$.
        \item Compute the Merkle root of $\{C_i'\}$. Let it be $r'$.
        \item Check if $r=r'$. If so, deliver $B'$. Otherwise, deliver \texttt{BAD\_UPLOADER}.
    \end{enumerate}
\end{itemize}

\vspace{10pt}
\underline{\textbf{\texttt{Retrieval}(K, r) handler at $i$-th node}}
\vspace{2pt}
\begin{itemize}
    \item Upon receiving \texttt{RequestChunk}$(K, r)$, the $i$-th server responds with \texttt{ReturnChunk}$(K, r, C_i, P_i)$.
\end{itemize}

} }
\caption{
Algorithm for \texttt{Retrieval}(K, r)
}
\label{fig:retrievalAlgo}
\end{figure}

\textbf{Retrieval algorithm} is formally defined in Figure~\ref{fig:retrievalAlgo}.
A client begins a retrieval by requesting chunks for the block with key $K$ from all nodes. Then, each node, if not byzantine, returns \texttt{ReturnChunk}$(K, r, C_i, P_i)$, where $i$ is the node index. The client checks the validity of the returned chunk by using Merkle proof $P_i$, Merkle root $r$, and the chunk content $C_i$. This should detect if a byzantine node returned a chunk that is different from the one originally encoded by the \texttt{Dispersal} invoker. Once the client collected $N - 2f$ or more valid chunks, it should be able to decode to recover the block content.

However, there's one potential vulnerability: if the original Dispersal invoker was byzantine, it could have built Merkle-tree with incorrect chunks not from the erasure coding (e.g., replacing $C_0$ and $C_1$ with something not from erasure coding). Such attacks may result in some nodes succeeding in the retrieval of the original block $B$ (if it decoded from $N-2f$ correct chunks) but other nodes retrieving wrong blocks (if its $N-2f$ set included an incorrect chunk). 

To detect the corrupted erasure coding by a byzantine uploader, a retriever, after decoding with $N-2f$ chunks, must re-encode the block with the same erasure coding mechanism. Then, by comparing the Merkle root values from the original uploader and re-encoding, the retriever can verify that the uploader followed the dispersal protocol, and every non-byzantine retriever will decode the same block. 

\subsubsection{Correctness of AVID-M}
\label{sec:avidm-correctness}
In this section, we analyze whether the AVID-M protocol satisfies the four properties mentioned in \S\ref{sec:avid-model}: termination, agreement, availability, and correctness.

For termination, all correct nodes must terminate when a correct client invoked \texttt{Disperse}(B, K). The correct client sends \texttt{Chunk} to all nodes, so all but byzantine ($N-f$) nodes will send out \texttt{GotChunk}. Subsequently, $N-f$ or more nodes should send out \texttt{Ready}. As $N-f \ge 2f+1$, all servers will terminate.

For agreement, all correct nodes must terminate as long as any correct one terminates, even if the uploading client was byzantine. This is
guaranteed by the fact that a server sends out \texttt{Ready} when it receives $f+1$ \texttt{Ready} messages from other servers, and terminates when it receives $2f+1$ \texttt{Ready} messages. As a result, when one server terminates, at least $f+1$ other correct servers have sent out \texttt{Ready} messages. This should drive all correct servers to send out \texttt{Ready}. So eventually, at least $N-f$ servers will send out \texttt{Ready}. As long as $N-f \ge 2f+1$,
all servers will terminate.

For availability, a correct server's termination must be sufficient to guarantee the retrieval by any correct client. In AVID-M, a correct server terminates only after it receives $2f+1$ \texttt{Ready} messages, among which $f+1$ must come from correct servers. A correct server sends out \texttt{Ready} for two reasons: receiving $N-f$ \texttt{GotChunk}'s, or receiving $f+1$ \texttt{Ready}'s. Since there are $f$ faulty servers, at least one correct server must have sent out \texttt{Ready} because of the first reason. It must have received $N-2f$ \texttt{GotChunk}'s from correct sources, each holding a chunk and a matching Merkle proof. A retrieving client can decode using these chunks. Regardless of the Merkel root check, the correct client will get either the original block or \texttt{BAD\_UPLOADER} (considered as a block for the proof).

For the correctness property, we should show that two clients will always deliver the same block, and we prove it by contradiction. Suppose that two correct clients running the retrieval protocol have decoded different blocks, $B_1$ and $B_2$. Because $B_1 \ne B_2$, when both clients re-encode the blocks, they will get different results. If neither encoding result matches the original Merkle root, then both clients should have rejected the retrieved blocks. 
Otherwise (without losing generality, assuming that the encoding result of $B_1$ matches the original Merkle root), the Merkle root correctly commits to the block $B_1$. Because $B_2$ is decoded from the chunks committed by the same Merkle root, we must have $B_1 = B_2$.
\red{What about B = B' when the uploader was honest?}


\subsection{Building Block 2: BA}
The second building block of DispersedLedger is Binary Agreement (BA). It allows $N-f$ correct servers to reach an agreement on a binary decision, where there are $f$ byzantine nodes among $N$ total nodes. 

BA has two primitives: \texttt{Input}($1$ or $0$) and \texttt{Output}() $\rightarrow$ (1 or 0). \texttt{Output} returns after at least $N-f$ has called \texttt{Input}.

A BA protocol provides the following properties:
\begin{itemize}
    \item \textbf{Agreement}: If any correct process outputs the bit $b$, then every correct process outputs $b$.
    \item \textbf{Termination}: If all correct processes receive input, then every correct process outputs a bit.
    \item \textbf{Validity}: If any correct process outputs $b$, then at least one correct process received $b$ as the input.
\end{itemize}

In this paper, we use an existing protocol~\cite{baprotocol} that completes in $O(1)$ time and the per-node communication cost is $O(N\lambda)$ where $\lambda$ is the security parameter. Binary Agreement should be a well-studied problem, so we may have other choices.


\subsection{DispersedLedger Protocol}
In this section, we discuss how to construct DispersedLedger from VID and BA. The construction is inspired by~\cite{acsconstruction} and
HoneyBadgerBFT. DispersedLedger runs in epochs; in each epoch, around $N$ blocks are committed. Each participating node proposes a block which consists of transactions sent from DispersedLedger clients, and proposals from well-behaving nodes are committed to the ledger.

We first describe the DispersedLedger protocol for a single epoch and then explain how to extend the protocol to multiple epochs so that each node can follow the bandwidth of its own without slowing down other nodes.

\subsubsection{Single Epoch Protocol}
\label{sec:design-singleEpoch}

Let the current epoch be $e$. On the $i$-th node, there is an input queue $Q_i$ that buffers the transactions submitted by clients. %
\footnote{In the SMR scenario, A client typically submits a transaction to a DispersedLedger node (preferably, the one it trusts), expecting the node will try to commit the transaction. In case of a server failure, the client may retry with other nodes, with the hope of hitting a not failed server eventually. This approach may result in duplicate transactions in blocks proposed by different nodes. We assume that the application layer can handle duplicate transactions and ensure the exactly-once semantics~\cite{rifl}.}

In each epoch, each DispersedLedger node participates in $N$ instances of VID and BA. Let $\text{VID}_j$ be the $j$-th ($j \in [N]$) VID instance for the block being dispersed from the $j$-th node. Let $\text{BA}_j$ be the $j$-th ($j \in [N]$) BA instance for agreeing on whether to commit the block being dispersed from the $j$-th node.

\begin{figure}
\centering
\fbox{%
  \parbox{0.95\columnwidth}{%

\underline{\textbf{Phase 1: Commitment on dispersed blocks}}
\vspace{2pt}
\begin{enumerate}
    \item Peek the front of $Q_i$ to get the next set of transactions (the block) $B_i$ to broadcast in epoch $e$. Let $H_i$ be the hash of the block.
    \item Run \texttt{Dispersal}$(B_i, H_i)$ as a client to kick off $\text{VID}_i$. \todo{fix: not $H_i$, it's an identifier, epoch\_num + node\_id.. should not allow impersonation.. Maybe change dispersal by Disperse($B_i$,invoker\_id,key)}
\end{enumerate}
\begin{itemize}
    \item Upon finishing $\text{VID}_j$ ($j \in [N]$), if an input has not been provided for $\text{BA}_j$, then input 1 to $\text{BA}_j$.
    \item Upon delivery of value 1 from at least $N-f$ BA instances, provide input 0 to all remaining BA instances that it has not provided an input.
    \item Upon delivery of value 1 from $BA_i$, remove the transactions in $B_i$ from $Q_i$.
    \item Upon termination of all BA instances,
    \begin{enumerate}
        \item let $S \subset [1 \dots N]$ be the indices of each BA instance that delivered 1.
        \item Move to phase 2.
    \end{enumerate}
\end{itemize}

\vspace{10pt}
\underline{\textbf{Phase 2: Lazy block retrieval}}
\vspace{2pt}
\begin{enumerate}
    \item Start responding to \texttt{GetChunk} messages for all VID instances.
    \item Run \texttt{Retrieval} of $\text{VID}_j$ ($j \in S, j \ne i$) to download the full blocks $B_j$ ($j \in S, j \ne i$).
    \item Deliver $\{B_j\}_{j \in S}$ (sorted by increasing indices) if we have delivered all previous epochs (up until $e-1$). Ignore messages that have been delivered before.
\end{enumerate}

} }
\caption{
Algorithm for single-epoch DispersedLedger
}
\label{fig:singleEpochAlgo}
\end{figure}

Figure~\ref{fig:singleEpochAlgo} describes the single epoch protocol for the $i$-th node. It begins by preparing a block proposal by collecting transactions from the input queue. The $i$-th node disperses the block proposal through $\text{VID}_i$. 

Because of $f$ potential byzantine failures, we cannot wait for all $N$ instances of VID to complete (note that the termination property of VID only guarantees termination if the invoker client was well-behaving). Thus, DispersedLedger uses $\text{BA}_i$ to reach an agreement on that $\text{VID}_i$ has been completed, so $\text{B}_i$ is considered to be committed in the current epoch. To do so, each server input 1 (meaning ``recommending to commit $B_i$'') for $\text{BA}_i$ once its $\text{VID}_i$ terminates. Once it learns that nodes have agreed on the commitment of $N-f$ blocks, it gives up on not-yet-dispersed blocks by providing input 0 to all remaining BA instances. In the meanwhile, if BA decided to commit $B_i$, the $i$-th node removes the transactions in $B_i$ from its input queue. Once all blocks are determined to be included or not in the current epoch, we move to phase 2.

In phase 2, a node starts to serve retrieval requests for blocks dispersed in the current epoch. It also retrieves all blocks committed in the current epoch, except the one proposed by itself as it already owns it. Once all retrievals are finished, a node delivers all committed blocks (sorted by increasing indices) to the application if all previous epochs are delivered.

\subsubsection{Inter-node Linking} 
\seojin{I don't see why this is called ``inter-node linking.'' No node commits the block proposed by other node. It gets committed by a consensus.}

We optimize the single epoch protocol described in \S\ref{sec:design-singleEpoch} for multi-epochs with a new technique called \textit{inter-node linking}. 

In the single epoch protocol in Figure~\ref{fig:singleEpochAlgo}, up to $f$ successfully dispersed blocks may be abandoned in each epoch. Since correct nodes input 0 to up to $f$ BA instances, the single epoch protocol may not commit up to $f$ blocks even if their VIDs are finished. This leads to two problems. First, in the worst case, almost one third of the network bandwidth used for phase 1 may be wasted. Second, a transaction $m$ submitted to a correct node may not be committed indefinitely. 

Our solution for the abandoned blocks is \textit{inter-node linking}, which is another mechanism for reaching an agreement on VID completions for \textit{previous} epochs (in contrast, BA is for current epochs). The key idea is that, by piggybacking each node's progress on VIDs of all previous epoch, correct nodes can reach a consensus on the completion of all VIDs of previous epochs. With that knowledge, correct nodes atomically deliver the blocks whose VID has been finished but not previously delivered (in addition to the blocks committed in the current epoch through BA).

With inter-node linking, each node now keeps two additional states. First, an integer array $V$ of size $N$ where $V[j]$ records the latest epoch for which, according to the knowledge of this node, all $\text{VID}_j$ has been finished in all previous epochs. Second, a 2-D boolean array $D$ where $D[j][e]$ records whether the block proposed in the epoch $e$ by the $j$-th node has been delivered or not.

At the beginning of each epoch, a node prepares its proposal block with its array $V$ in addition to the set of transactions so that $V$ can be dispersed and retrieved as well. Once the commit phase completes, there are $N-f$ or more such $V$ arrays are committed and available for retrieval. 

Upon retrieving all blocks whose BA outputs are 1, a node computes the completion of VIDs of previous epochs. For each \texttt{Dispersal} invoker $j$, the node takes the $f+1$-largest epoch number from the $2f+1$ (or more) $V$ arrays; the result indicates the completion of $\text{VID}_j$ at least until the $f+1$-largest epoch. By taking $f+1$-largest epoch, we tolerate $f$ byzantine nodes reporting wrong $V$'s. Also, taking the largest epoch among the guaranteed to be correct $V$ is okay thanks to the agreement property of VID (once finished by a correct node, a VID instance will finish at all other correct nodes eventually). Finally, all correct nodes will get the same result as nodes exchanged $V$ through the atomic broadcast of the current epoch.

With the agreed view on VID completions in previous epochs, nodes check if any blocks that was dispersed by not yet delivered by referring its $D$. Nodes retrieve such blocks and deliver them after the blocks proposed and committed in the current epoch. For atomic broadcast, nodes sort such blocks by a tuple <epoch\_of\_proposal, proposer\_id>. 

The formal protocol updated from Figure~\ref{fig:singleEpochAlgo} is in Appendix~\ref{sec:appendix-internodeLinking}.





\subsubsection{Running Multiple Epochs in Parallel}

In DispersedLedger, a node runs the first phase of each epoch sequentially. Globally, phase 1 of epochs proceeds sequentially with less than $f$ nodes may fall behind at older epochs.

On the other hand, the second phase of each epoch runs independently in parallel. We not only decouple the commitment phase from the lazy retrieval phase, each retrieval independently except the final delivery to the application, which must be sequential to provide the total order.

The benefit of running retrievals across epochs is maximizing network utilization. Since DispersedLedger nodes transfer data among them, a node may not fully utilize its ingress bandwidth if the sources of the requested chunks are short of egress bandwidth. By trying to download blocks of any epochs whose Phase 1 was completed, a node can increase the number of senders and avoid getting bottlenecked by the sender's egress bandwidth, resulting in maximizing the utilization of its ingress bandwidth.

However, this aggressive approach potentially interferes with the transmission of messages for higher priority tasks, such as phase 1 or the retrieval of earlier epochs. To minimize the interference and prevent slowing down phase 1, we prioritize VID traffic over retrieval traffic, and retrievals of the lowest epoch over higher epochs. Such prioritization is possible on the Internet with standard networking hardware and standard transports, such as QUIC. \S\ref{sec:impl-priority} discusses how to implement such prioritization.

\todo{discuss about the corner case where there is a very fast node and only this fast node can retrieve. Just discuss about possible solutions. Important because in the real world the bw distribution has a long tail. This is a policy decision. In the most cases, you would still want some limit.}

\subsection{Correctness of DispersedLedger}
We now informally analyze the correctness of the DispersedLedger protocol by showing that it guarantees the four properties required for atomic broadcast protocols, which were introduced in \S\ref{sec:design-model}.

First, both of our building blocks, VID and BA, tolerates $f$ byzantine faults on asynchronous network.

\textbf{Agreement.} Let's backtrace how a correct node (say $n$) delivered the message $m$. For the message $m$ to be delivered at a node $n$, the block (say $B_j$) that packed should have been included in $S$, the set of blocks with $\text{BA}_j$ output of 1. By the agreement property of BA, $\text{BA}_j$ at all correct nodes should have output 1 as well. Thus, every correct node includes $B_j$ in $S$ and will try to retrieve the block $B_j$. By the availability property of VID, every correct node can retrieve a block $B_{j}'$. By the correctness property of VID, the block being delivered must be same as $B_j$ and include $m$. As all correct nodes must also deliver $m$ eventually, we satisfied the agreement property.

\textbf{Total order.} As we just analyzed for agreement, every correct node should have the same $S$ (thanks to BA's agreement property) for every epoch. Since each node sort blocks in $S$ by proposers' indices, the history of delivered blocks must be same across all correct nodes.

\textbf{Liveness.\ly{Validity?}} \redstrike{when a client submits a message $m$ to $N-f$ correct nodes, at least one of the correct node (say $n_j$) should succeed at $\text{BA}_j$. By the termination property of VID,  all $N-f$ correct nodes will eventually finish the VID instances invoked by themselves. However, if the VIDs invoked by $f$ byzantine nodes finish earlier, correct nodes may input 0 to at most $f$ BA instances for the blocks proposed by correct nodes. Considering $f$ byzantine nodes may input 0 to arbitrary BA instances, there are at most $f$ * $N$ input 0's; as each BA instance needs more than half inputs to be input 0 to get output 0, we may get at most $2f$ BA instances with output 0. \todo{fix} As $N = 3f+1$, we have $2f+1$ BA instances from correct nodes, so there must be at least one BA instance with output 1 from $N-f$ correct node. Through the block proposed by the correct node, all correct nodes deliver the message $m$.}

\subsection{Outline - keep it for now}
\subsubsection{Protocol}






\textbf{Prioritization.} \todo{First, why and how to prioritize high-priority traffic. Actually prioritization does not help much in our case because the available bandwidths are always higher than VID bandwidth. Still, explain that we modify Cubic to achieve prioritization. Also say that it is not being unfair to other flows: we are just sending at a very low rate.} \seojin{talk about this in implementation?}

\todo{Second, importance of ordering between rounds. The system should deliver round 1 data before round 2 data. Note that this does not need to be strict. According to our observation best-effort ordering is enough. If we have space and time maybe show a counterexample.}

\textbf{Infinite pipelining.} \todo{Because it does not make much sense to deliberately throttle proposal. As a result, slow nodes can still propose even if they can't download all the data. Note that it does not mean that the system loses backpressure: they are still backpressure the users (those who want to send transactions) by looking at number of rounds proposed vs retrieved.}

\textbf{Inter-node linking.} \todo{HB solves censorship using threshold encryption. Turns out that there is a much better way to do this - inter-node linking. Benefit 1: no block will be wasted (maybe show some figures to prove). Benefit 2: no computational overhead.}

